Indefinite causal order with output-signalling instruments

Quantum processes can exhibit indefinite causal order, allowing coherent superpositions of distinct orderings of events. Whether such processes generate genuinely noncausal statistics, however, depends not only on their global causal structure but also on the local operations available to the parties. Here, we restrict communication to the classical outcomes of local operations, yielding a causal polytope with new causal inequalities that can be violated using measure-and-reprepare, entanglement-breaking instruments requiring no coherent transmission through the laboratories. Using a semidefinite-programming framework, we bound the achievable violations and reveal noncausal correlations that satisfy all conventional input-signalling inequalities, demonstrating that restricting the information available for communication can uncover forms of indefinite causal order inaccessible under less restrictive operational assumptions.

==> images/inp_sing_dags.tex <==
\begin{figure}[ht!]
\centering

\caption{\textmd{DAGs representing scenarios of input communication between two parties, A and B, with common a source $\Lambda$.}}
\label{fig:inp_sing_dags}
% \fcolorbox{gray}{white}{\includegraphics[width=0.8\textwidth]{images/inp_sing_dags.png}}
\includegraphics[width=0.5\textwidth]{images/inp_sing.png} 

% \par\medskip\ABNTEXfontereduzida\selectfont\textbf{Source:} \citeauthoronline{shanenkoNF2007} (\citeyear{shanenkoNF2007}) \par\medskip
\end{figure}

==> images/out_sing_dags.tex <==
\begin{figure}[ht!]
\centering

\caption{\textmd{DAGs representing scenarios of output communication between two parties, A and B, with common a source $\Lambda$. }}
\label{fig:out_sing_dags}
% \fcolorbox{gray}{white}{\includegraphics[width=0.8\textwidth]{images/out_sing_dags.png}}
\includegraphics[width=0.5\textwidth]{images/out_sing.png}



% \par\medskip\ABNTEXfontereduzida\selectfont\textbf{Source:} \citeauthoronline{shanenkoNF2007} (\citeyear{shanenkoNF2007}) \par\medskip
\end{figure}

==> new_inequalities.tex <==
\begin{align}
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 2 p(01\vert01) + 2 p(11\vert01) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) + 1 p(10\vert11) &\leq 2 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 2 p(01\vert01) + 2 p(11\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(10\vert00) + 1 p(11\vert00) + 2 p(00\vert01) + 1 p(01\vert01) + 2 p(10\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(10\vert00) + 1 p(11\vert00) + 2 p(00\vert01) + 1 p(01\vert01) + 2 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(01\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(10\vert00) + 1 p(11\vert00) + 2 p(00\vert01) + 2 p(01\vert01) + 1 p(11\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 2 p(00\vert11) + 2 p(10\vert11) &\leq 2 \\
    1 p(10\vert00) + 1 p(11\vert00) + 2 p(00\vert01) + 2 p(01\vert01) + 2 p(11\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) &\leq 2 \\
    1 p(10\vert00) + 1 p(11\vert00) + 2 p(00\vert01) + 2 p(01\vert01) + 2 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(01\vert11) + 1 p(11\vert11) &\leq 2 \\
    2 p(10\vert00) + 2 p(11\vert00) + 1 p(00\vert01) + 2 p(01\vert01) + 2 p(11\vert01) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) &\leq 2 \\
    2 p(10\vert00) + 2 p(11\vert00) + 2 p(00\vert01) + 1 p(01\vert01) + 2 p(10\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(01\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(01\vert00) + 1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 2 p(01\vert11) + 2 p(10\vert11) + 2 p(11\vert11) &\leq 2 \\
    1 p(01\vert00) + 1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(01\vert11) + 2 p(10\vert11) + 2 p(11\vert11) &\leq 2 \\
    1 p(01\vert00) + 1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(01\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(01\vert00) + 1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(10\vert01) + 2 p(00\vert10) + 2 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) &\leq 2 \\
    1 p(01\vert00) + 2 p(10\vert00) + 2 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 2 p(00\vert10) + 2 p(10\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(01\vert00) + 2 p(10\vert00) + 2 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(11\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(00\vert00) + 1 p(10\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(11\vert01) + 2 p(00\vert10) + 2 p(01\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(00\vert00) + 1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(11\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 2 \\
    1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(01\vert01) + 1 p(11\vert01) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(01\vert01) + 1 p(11\vert01) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) &\leq 1 \\
    1 p(01\vert01) + 1 p(11\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(01\vert01) + 1 p(11\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(11\vert10) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(01\vert01) + 1 p(10\vert01) + 1 p(11\vert01) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) &\leq 1 \\
    1 p(00\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(01\vert11) &\leq 1 \\
    1 p(00\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(01\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(00\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(00\vert01) + 1 p(10\vert01) + 1 p(11\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(01\vert11) &\leq 1 \\
    1 p(00\vert01) + 1 p(01\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert11) &\leq 1 \\
    1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(00\vert11) + 1 p(01\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(00\vert10) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(00\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(01\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(00\vert11) + 1 p(10\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(01\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(01\vert01) + 1 p(11\vert01) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(01\vert01) + 1 p(11\vert01) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(00\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(01\vert11) + 1 p(11\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(10\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(11\vert10) + 1 p(01\vert11) &\leq 1 \\
    1 p(10\vert00) + 1 p(11\vert00) + 1 p(00\vert01) + 1 p(01\vert01) + 1 p(00\vert10) + 1 p(10\vert10) + 1 p(00\vert11) + 1 p(10\vert11) &\leq 1 \\
    1 p(11\vert11) &\leq 0 \\
    1 p(10\vert11) &\leq 0 \\
    1 p(00\vert11) &\leq 0 \\
\end{align}
